On the Uniqueness of Fr\'echet Means for Polytope Norms

Fr\'echet means are a popular type of average for non-Euclidean datasets, defined as those points that minimise the average squared distance to a set of data points. We consider the behaviour of sample Fr\'echet means on normed spaces whose unit ball is a polytope; this setting is particularly important for semi-discrete data, but is rarely covered by existing literature on Fr\'echet means, which focuses primarily on manifolds and spaces with bounded Alexandrov curvature. We study the geometry of the set of Fr\'echet means over polytope normed spaces, with a focus on dimension and probabilistic conditions for uniqueness. In particular, we provide a geometric characterisation of the threshold sample size at which Fr\'echet means have a positive probability of being unique, and we prove that this threshold is at most one more than the dimension of our space. This geometric characterisation presents a novel framework for computing the unique Fr\'echet mean sample threshold, which we demonstrate in the case of the $\ell_1$, $\ell_{\infty}$ and tropical norms. In particular, we show that the $\ell_1$ sample threshold is always 3, but the $\ell_{\infty}$ and tropical sample thresholds grow at different rates with the dimension of our space.

==> Preamble.tex <==
\usepackage{url}\RequirePackage[colorlinks,citecolor=blue, linkcolor=blue,urlcolor = blue]{hyperref}
\usepackage{latexsym,amssymb,amsmath,amsfonts,graphicx,color,fancyvrb,enumerate,subcaption,mathrsfs}
\usepackage{amsthm}
\usepackage[longnamesfirst,authoryear,round]{natbib}
\usepackage{xy}\xyoption{all} \xyoption{poly} \xyoption{knot}
\usepackage{float}
\thispagestyle{empty} % no page number on front page
\usepackage{bm}
\usepackage{booktabs}
\usepackage{diagbox}
\usepackage{bbm}
\usepackage{placeins}
\usepackage{multicol,multirow}
\usepackage[safe]{tipa}
\usepackage{array}
\usepackage{relsize}
\usepackage{chngcntr}
\usepackage{etoolbox}
\usepackage{caption}
\usepackage{tikz}
\usetikzlibrary{patterns}
%\usetikzlibrary{math}
\usepackage{tikz-3dplot}
\usetikzlibrary{decorations.pathreplacing,calc}
\usetikzlibrary{shapes,backgrounds}
\usetikzlibrary{patterns}
\usetikzlibrary{cd}
\usepackage{amsopn}
\usepackage{calc}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage{hyperref}
\usepackage{mathtools}
\newcommand{\indep}{\rotatebox[origin=c]{90}{$\models$}}
\usepackage{tikz-cd} % commutative diagrams
\usepackage{amscd} % commutative diagrams
\usepackage{comment}
\usepackage[capitalize,nameinlink,compress]{cleveref}
\crefname{figure}{Figure}{Figures} 
\crefname{equation}{}{} 
\crefname{assumption}{Assumption}{Assumptions}
\crefname{subsection}{Subsection}{Subsections}
\usepackage{textcomp}
\usepackage{mathabx}
\usepackage{thmtools}
\usepackage{thm-restate}

\newcounter{cdrow}
\newcommand\cdlabel[1]{%
  \Crefstepcounter{cdrow}
  \label{#1}
  (\thecdrow)
}

%%% Formatting theorems
\newtheorem{theorem}{Theorem}[section]
\newtheorem*{theorem*}{Theorem}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{claim}[theorem]{Claim}
\newtheorem*{claim*}{Claim}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem*{definition*}{Definition}
\newtheorem{assumption}{Assumption}
\newtheorem{question}{Question}


\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{remarks}[theorem]{Remarks}
\newtheorem{example}[theorem]{Example}
\newtheorem*{example*}{Example}

\DeclareMathOperator{\tr}{tr}


% custom definitions ...
\def\eq#1{(\Cref{#1})}
\def\pdf{p.d.f.\ } \def\cdf{c.d.f.\ }
\def\pdfs{p.d.f.s} \def\cdfs{c.d.f.s}
\def\mgf{m.g.f.\ } \def\mgfs{m.g.f.s\ }
\def\ci{\perp   \perp}  % conditional independence symbol
\def\diag{{\rm diag}}
\def\log{{\rm log}}
\def\tr{{\rm tr}}
\def\cond{\, | \,}
\newcommand\myeq{\stackrel{\mathclap{\normalfont\mbox{$t := r^p$}}}{=}}
\newcommand*\diff{\mathop{}\!\mathrm{d}}

\makeatletter
\newcommand*{\op}{%
  \DOTSB
  \mathop{\vphantom{\bigoplus}\mathpalette\matt@op\relax}%
  \slimits@
}
\newcommand\matt@op[2]{%
  \vcenter{\m@th\hbox{\resizebox{\widthof{$#1\bigoplus$}}{!}{$\boxplus$}}}%
}
\makeatother

\def\dsum{\displaystyle\sum}
\def\dint{\displaystyle\int}
\def\dsup{\displaystyle\sup}
\def\dinf{\displaystyle\inf}
\def\dmin{\displaystyle\min}
\def\dlim{\displaystyle\lim}
\def\bz{{\mathbf z}} % sample

\newcommand{\comp}{\mathbb{C}}
\newcommand{\sph}{\mathbb{S}}
\newcommand{\bola}{\mathbb{B}}
\newcommand{\disk}{\mathbb{D}}

\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Ebb}{\mathbb{E}}
\newcommand{\Fbb}{\mathbb{F}}
\newcommand{\Kbb}{\mathbb{K}}
\newcommand{\Lbb}{\mathbb{L}}
\newcommand{\Mbb}{\mathbb{M}}
\newcommand{\Vbb}{\mathbb{V}}
\newcommand{\Xbb}{\mathbb{X}}
\newcommand{\Ybb}{\mathbb{Y}}
\newcommand{\Zbb}{\mathbb{Z}}

\newcommand{\prt}{\partial}

\newcommand{\Ker}{\mathrm{Ker} \,}
\renewcommand{\Im}{\mathrm{Im} \,}
\newcommand{\Coker}{\mathrm{Coker} \,}
\renewcommand{\H}{\mathrm{H}}
\newcommand{\rank}{\mathrm{rank} \,}
\renewcommand{\L}{\mathcal{L}}


\newcommand{\abf}{\mathbf{a}}
\newcommand{\cbf}{\mathbf{c}}
\newcommand{\fbf}{\mathbf{f}}

\newcommand{\VR}{\mathrm{VR}}

\newcommand{\ot}{\mathrm{OT}}
\newcommand{\T}{\intercal}
\newcommand{\Trop}{\mathrm{Trop}}
\newcommand{\Sym}{\mathrm{Sym}}
\newcommand{\argmin}{\text{argmin}}
\newcommand{\argmax}{\text{argmax}}
\newcommand{\codim}{\textrm{codim}}
\newcommand{\TPT}[1]{ \R^{#1}/\R \mathbf{1}}
\newcommand{\norm}[2]{\Vert #2 \Vert_{#1}}
\newcommand{\dtr}{d_{\mathrm{tr}}}
\newcommand{\esssupp}{\mathrm{esssupp}}
\newcommand{\CType}{F_1,\dots,F_n}
\newcommand{\sample}{\vec X_1,\dots, \vec X_n}
\DeclareMathOperator{\tconv}{tconv}
\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\relint}{relint}
\DeclareMathOperator{\closure}{Cl}
\DeclareMathOperator{\FMset}{\mathcal{F}}
\DeclareMathOperator{\aff}{aff}
\DeclareMathOperator{\proj}{proj}


\newcommand{\am}[1]{{\textcolor{cyan}{ #1  --Anthea}}} %%% Added by Anthea. For comments to appear in manuscript.
\newcommand{\rt}[1]{ {\textcolor{violet!60!magenta}{ #1  --Roan.}}} %%% Roan's comments
\newcommand{\amc}[1]{ {\textcolor{orange}{ #1  --Andy.}}} %%% Andy's comments

% \newcommand{\bigboxplus}{
%   \mathop{
%     \vphantom{\bigoplus} 
%     \mathchoice
%       {\vcenter{\hbox{\resizebox{\widthof{$\displaystyle\bigoplus$}}{!}{$\boxplus$}}}}
%       {\vcenter{\hbox{\resizebox{\widthof{$\bigoplus$}}{!}{$\boxplus$}}}}
%       {\vcenter{\hbox{\resizebox{\widthof{$\scriptstyle\oplus$}}{!}{$\boxplus$}}}}
%       {\vcenter{\hbox{\resizebox{\widthof{$\scriptscriptstyle\oplus$}}{!}{$\boxplus$}}}}
%   }\displaylimits 
% }


\newcommand{\ms}[1]{\mathscr{#1}}
\newcommand{\sgn}{\text{\sgn}}
\newcommand{\Vol}{\text{Vol}}
\newcommand{\one}{1}
\newcommand{\two}{2}
\newcommand{\id}{\text{id}}
\newcommand{\supp}{\text{Supp}}
\newcommand{\Poi}{\text{Poi}}
\newcommand{\Tan}{\text{Tan}}
\newcommand{\diam}{\text{diam}}
\newcommand{\Prob}{\mathbb{P}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\W}{\mathcal{W}}
\renewcommand{\P}{\mathcal{P}}
\renewcommand{\vec}[1]{\mathbf{#1}}
\newcommand{\trop}{\text{trop}}
\newcommand{\im}{\text{Im}}
\renewcommand{\ker}{\text{Ker}}
\newcommand{\Cov}{\text{Cov}}
\newcommand{\Var}{\text{Var}}
\DeclareMathOperator{\type}{type}
\newcommand{\bl}[1]{{\mathbf #1}}
\newcommand{\bs}[1]{\boldsymbol #1}
\newcommand{\mb}[1]{\mathbb #1}
\newcommand{\mc}[1]{\mathcal #1}
\newcommand{\NR}{\mathcal{N}\mathcal{R}}
\newcommand{\A}{\mathcal{A}}

\makeatletter
\def\@biblabel#1{}
\makeatother

\makeatletter
\patchcmd{\NAT@citex}
  {\@citea\NAT@hyper@{%
     \NAT@nmfmt{\NAT@nm}%
     \hyper@natlinkbreak{\NAT@aysep\NAT@spacechar}{\@citeb\@extra@b@citeb}%
     \NAT@date}}
  {\@citea\NAT@nmfmt{\NAT@nm}%
   \NAT@aysep\NAT@spacechar\NAT@hyper@{\NAT@date}}{}{}

% Patch case where name and year are separated by opening bracket
\patchcmd{\NAT@citex}
  {\@citea\NAT@hyper@{%
     \NAT@nmfmt{\NAT@nm}%
     \hyper@natlinkbreak{\NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi}%
       {\@citeb\@extra@b@citeb}%
     \NAT@date}}
  {\@citea\NAT@nmfmt{\NAT@nm}%
   \NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi\NAT@hyper@{\NAT@date}}
  {}{}

\makeatother
